Parallel In-Place Algorithms: Theory and Practice

Many parallel algorithms use at least linear auxiliary space in the size of the input to enable computations to be done independently without conflicts. Unfortunately, this extra space can be prohibitive for memory-limited machines, preventing large inputs from being processed. Therefore, it is desirable to design parallel in-place algorithms that use sublinear (or even polylogarithmic) auxiliary space. In this paper, we bridge the gap between theory and practice for parallel in-place (PIP) algorithms. We first define two computational models based on fork-join parallelism, which reflect modern parallel programming environments. We then introduce a variety of new parallel in-place algorithms that are simple and efficient, both in theory and in practice. Our algorithmic highlight is the Decomposable Property introduced in this paper, which enables existing non-in-place but highly-optimized parallel algorithms to be converted into parallel in-place algorithms. Using this property, we obtain algorithms for random permutation, list contraction, tree contraction, and merging that take linear work, $O(n^{1-\epsilon})$ auxiliary space, and $O(n^\epsilon\cdot\text{polylog}(n))$ span for $0<\epsilon<1$. We also present new parallel in-place algorithms for scan, filter, merge, connectivity, biconnectivity, and minimum spanning forest using other techniques. In addition to theoretical results, we present experimental results for implementations of many of our parallel in-place algorithms. We show that on a 72-core machine with two-way hyper-threading, the parallel in-place algorithms usually outperform existing parallel algorithms for the same problems that use linear auxiliary space, indicating that the theory developed in this paper indeed leads to practical benefits in terms of both space usage and running time.

==> figure-rp-exp.tex <==
\begin{figure*}[t]
%\vspace{-1em}
\begin{center}
  \includegraphics[width=.9\columnwidth]{data/1}
  \includegraphics[width=.9\columnwidth]{data/2}
\end{center}\vspace{-1.2em}
\caption{\normalfont The actual running times (left) and relative running times compared to \algname{RP-PBBS} (right) of different implementations for random permutation on  72 cores with hyper-threading.  The input size varies from 10 million to 1 billion integers.
  %The running times in the right figure is normalized to \algname{RP-PBBS}.
}
%\vspace{-2em}
\label{fig:rp-exp}
\end{figure*}




==> figure-scan.tex <==
\begin{figure*}[t]
\vspace{-1em}
\begin{center}
  \includegraphics[width=.7\columnwidth]{data/scan-time}
  \includegraphics[width=.7\columnwidth]{data/scan-scale}
\end{center}%\vspace{-1.2em}
%\vspace{-1.2em}
\caption{\small The left figure shows the running time of the in-place scan and PBBS scan when the input size varies from 10 million to 200 million. The right figure shows the relative speedup compared to sequential PBBS scan, when the input size is 100 million and the core count varies from 1 to 72 with hyperthreading.  In both cases the relative performance between in-place scan and PBBS scan is consistent.}
%\vspace{-2em}
\label{fig:scan-exp}
\end{figure*}




==> frt-pseudo.tex <==
\begin{algorithm2e}[!tp]
\caption{The ROSE FRT algorithm}
\label{algo:ROSE-FRT}
\SetKwFor{ParForEach}{parallel foreach}{do}{endfch}
\SetKwFor{ParFor}{parallel for}{do}{endfch}
\SetKw{break}{Break}
\KwIn{A graph $G=(V,E)$  with $V = \{v_1,\ldots,v_n\}$}
\KwOut{An FRT tree $T_{\pi,\beta}$}
\medskip
    Uniformly randomly permute the vertices in $G$ based on $\pi:V\rightarrow V$.\\
    Pick $\beta\in[1,2]$ with the probability density function $f_B(x)=1/(x\ln 2)$.\\
\medskip
We will maintain across the rounds the following:\\
\parbox{.45\textwidth}{
\begin{enumerate}
  \item A partial FRT tree (i.e., the top part).  Initially just a root
    node and finally the full tree.
  \item For $v \in V$, $\tau_v$ is a pointer to a leaf of the
    partial FRT which $v$ will eventually fall under (recall every
    vertex is a leaf of the final FRT tree).  Initially all point to the root.
  \item
    For $v \in V$, $\delta(v)$ is the smallest distance to $v$
    from vertices processed so far.   Initially $+\infty$.
  \end{enumerate}
  }\\
    \For{\upshape $r\gets 1$ to $\log_2 n$\label{line:prose-loop-r}} {
    \ParForEach{\upshape $i \in \{{2^{r-1},\ldots, 2^r-1}\}$\label{line:FRT-batch}} {
       Let $S_i=\{u \in V~|~d(v_i,u)<\delta(u)\}$\label{line:prose-sssp}
     }
    \ParForEach{$u \in V$\label{line:convert-start}}{
        Let $l(u)\gets \{\langle v_i, \rho_i=\lfloor
        \log_2{\frac{\beta\Delta}{d_G(v_i,u)}}\rfloor\rangle : 1 \leq
        i \leq n ~|~ u\in S_i\}$\\
        Sort $l(u)$ based on $\rho_i$ in descending order and filter out $v_i$ that are not in ascending order\\
      }
      Now collect vertices together using $\langle \tau_u,
      l(u)\rangle$, and just keep one of each equivalence class, and
      call the resulting set $\bar{S}$. \laxman{Can we clarify what
      equivalence class means? I think it's just remove duplicates?
      $\tau_u$ is also defined after this use in the next line.} Can
      be done with a semisort.  \label{line:FRT-semisort-locate}\\
      \ParForEach{$u \in \bar{S}$}{
        %\guy{Not sure why you are separating out the last one?}\\
        Let $\tau_u$ be the current tree node for $u$, and $l'_{(j)}(u)\gets \{\langle v_{u_1}, \rho_{u_1}\rangle,\ldots,\langle v_{u_{j-1}}, \rho_{u_{j-1}}\rangle, v_{u_{j}}\} ~|~ 1\le j\le |l(u)|$
        \laxman{Why is $(j)$ in the subscript for $l'(u)$? Should the
        end bounds be $j$ instead of $|l(u)|$ and the loop variable be
        $k$?}
      }
      For all $u \in \bar{S},j\le |l(u)|$, using a semisort collect together based  on
      key $\langle \tau_u, l'_{(j)}(u)\rangle$ along with value $\rho_{u_{j}}$.
      \label{line:FRT-semisort-group}\\
    \ParForEach{\upshape key $\langle \tau_u, l'_{(j)}(u)\rangle$
      after semisort}{
      % \guy{Didn't we already sort on line 10?}
      Sort the value $\rho_{u_j}$ in increasing order\\
      % \guy{I imagine this is trying to avoid having a single child,
      %   but since happening in parallel how do we know if there are
      %   others with the same $\tau_u$?}\\
      \If {\upshape $\tau_u$ has children} {
        Create a tree node for the first entry\label{line:FRT-create-case-1}
      }
      Create a tree node for every but the first entry, point the root of each node to the predecessor\label{line:FRT-create-case-2}
    }
    \ParForEach{$u \in \bigcup_i S_i$}{
        Point $u$ to the current corresponding node \label{line:convert-end}
      }
      For $v \in V$ update $\tau_v$ to point to new leaf.
    }
\end{algorithm2e}


==> table-all.tex <==
%\begin{table}[htbp]
\begin{minipage}[t]{0.45\textwidth}
  \small
  \centering
    \begin{tabular}{crrrr}
    \toprule
    \multicolumn{1}{c}{Input Size} & \multicolumn{2}{c}{Scan} & \multicolumn{2}{c}{Filter} \\
    \multicolumn{1}{c}{(million)} & \multicolumn{1}{c}{PBBS} & \multicolumn{1}{c}{PIP} & \multicolumn{1}{c}{PBBS} & \multicolumn{1}{c}{PIP} \\
    \midrule
    100   & 29    & 23    & 23    & 19 \\
    200   & 50    & 39    & 43    & 36 \\
    500   & 120   & 89    & 111   & 89 \\
    1000  & 250   & 170   & 215   & 172 \\
    2000  & 459   & 336   & 422   & 335 \\
    \bottomrule
    \end{tabular}%
  \caption{\normalfont Running times (in milliseconds) of the PBBS algorithms and the new PIP algorithms for scan and filter on 72 cores with hyper-threading.}
  \label{tab:addlabel}%
%\end{table}%

\bigskip

%\begin{table}[htbp]
\centering

    \begin{tabular}{crrrr}
    \toprule
    \multicolumn{1}{c}{Core} & \multicolumn{2}{c}{Scan} & \multicolumn{2}{c}{Filter} \\
    \multicolumn{1}{c}{count} & \multicolumn{1}{c}{PBBS} & \multicolumn{1}{c}{PIP} & \multicolumn{1}{c}{PBBS} & \multicolumn{1}{c}{PIP} \\
    \midrule
    1     & 3150  & 4170  & 2770  & 2150 \\
    4     & 1020  & 1230  & 861   & 701 \\
    8     & 548   & 630   & 524   & 393 \\
    18    & 308   & 331   & 301   & 244 \\
    36    & 280   & 255   & 254   & 191 \\
    72    & 265   & 192   & 222   & 179 \\
    72HT  & 250   & 170   & 215   & 172 \\
    \bottomrule
    \end{tabular}%
  \caption{\normalfont Running times (in milliseconds) of the PBBS algorithms and the new PIP algorithms for scan and filter on varying core counts.}
  \label{tab:addlabel}%
%\end{table}%

\bigskip

%\begin{table}%
   \begin{tabular}{cccccc}
    \toprule
    Output fraction &  12.5\% & 25\%   & 50\%   & 75\% & 87.5\% \\
    PBBS filter & 189   & 202   & 215   & 234 & 252 \\
    PIP filter  & 94    & 118   & 172   & 212 & 254 \\
    \bottomrule
    \end{tabular}%
  \caption{\normalfont Running times (in milliseconds) of the PBBS filter and the new PIP filter algorithms, with varying output fraction on 72 cores with hyper-threading.  The input is 1 billion integers.\label{tab:filter-fraction}}
%\end{table}%
\end{minipage}
\hspace{2em}
\begin{minipage}[t]{0.45\textwidth}
  \small
%\begin{table}[t]
  \centering
    \begin{tabular}{crrrrrr}
    \toprule
    Input Size & \multicolumn{3}{c}{List contraction} & \multicolumn{3}{c}{Tree contraction} \\
    (million) & &\multicolumn{1}{c}{PBBS} & \multicolumn{1}{c@{}}{PIP} & & \multicolumn{1}{c}{PBBS} & \multicolumn{1}{c@{}}{PIP} \\
    \midrule
    10   & & 59    & 49   & & 73    & 46 \\
    20   & & 79    & 70   & & 141   & 82 \\
    50   & & 142   & 131  & & 323   & 198 \\
    100  & & 247   & 205  & & 600   & 350 \\
    200  & & 494   & 418  & & 1170  & 680 \\
    \bottomrule
    \end{tabular}%
  \caption{\normalfont Running times (in milliseconds) of the PBBS algorithms and the new PIP algorithms for list and tree contraction on 72 cores with hyper-threading.}
  \label{tab:lt-runtime}%
%\end{table}%

\bigskip

%\begin{table}[t]
  \centering
    \begin{tabular}{crrrrrr}
    \toprule
    Core & \multicolumn{3}{c}{List contraction} & \multicolumn{3}{c}{Tree contraction} \\
    count & &\multicolumn{1}{c}{PBBS} & \multicolumn{1}{c@{}}{PIP} & & \multicolumn{1}{c}{PBBS} & \multicolumn{1}{c@{}}{PIP} \\
    \midrule
    1    & & 13900 & 3350  & & 22800 & 12600 \\
    4    & & 4370  & 1110  & & 8020  & 4370 \\
    8    & & 2180  & 636   & & 3950  & 2210 \\
    18   & & 1010  & 384   & & 2060  & 1220 \\
    36   & & 592   & 302   & & 1390  & 1050 \\
    72   & & 362   & 220   & & 899   & 512 \\
    72HT & & 247   & 205   & & 603   & 350 \\
    \bottomrule
    \end{tabular}%
  \caption{\normalfont Running times (in milliseconds) of the PBBS algorithms and the new PIP algorithms for list and tree contraction on varying core counts.}
  \label{tab:lt-scale}%
  
\bigskip

  \begin{tabular}{@{  }>{\centering}p{2.4cm}@{  }>{\centering}p{1.35cm}>{\centering}p{1.6cm}p{1cm}<{\centering}}
    \toprule
    Problem & Input size (MB) & Memory usage (MB) & Over-head \\
    \midrule
    Scan  & 7629.4 & 7636.2 & <0.1\% \\
    Filter & 7629.4 & 7636.9 & <0.1\% \\
    RandPerm & 762.9 & 791.2 & 3.7\% \\
    ListContraction & 762.9 & 773.5 & 1.4\% \\
    TreeContraction & 1144.4 & 1154.9 & 0.9\% \\
    \bottomrule
    \end{tabular}%
  \caption{\normalfont Memory usage of the five instances shown in \cref{fig:summary}.}
  \label{tab:memory-usage}%
  
\end{minipage}



%\end{table}%



==> table-rp.tex <==
\begin{minipage}[t]{0.47\textwidth}
  \small
    \centering
    \begin{tabular}{lrrrrr}
    \toprule
       Input size: & \multicolumn{1}{l}{10M} & \multicolumn{1}{l}{30M} & \multicolumn{1}{l}{100M} & \multicolumn{1}{l}{300M} & \multicolumn{1}{l}{1000M} \\
    \midrule
    \algname{RP-PBBS}  & 43.7  & 89.2  & 283   & 781   & 2680 \\
    \naive{} & 134   & 256   & 910   & 2580  & 9330 \\
    \rpflat{} & 98.1    & 187   & 644   & 1880  & 6280 \\
    \oneres{} & 77.1  & 133   & 422   & 1370  & 5250 \\
    \final{} & 65.6  & 131   & 388   & 1160  & 3960 \\
    \bottomrule
    \end{tabular}%
  \caption{\normalfont Running time (in milliseconds) of the five implementations of random permutation on 72 cores with hyper-threading.}
  \label{tab:rp-runtime}%
  \end{minipage}
  \hspace{1em}
  \begin{minipage}[t]{0.45\textwidth}
    \small
  \centering
    \begin{tabular}{lccc}
    \toprule
    Phase: & Reserve  & Commit  & Cleaning  \\
    \midrule
    \algname{RP-PBBS}  & 2/1  & 2/1  & 0/0 \\
    \naive{} & 0/3  & 0/3  & 3/0 \\
    \rpflat{} & 1/2  & 1/2  & 2/0 \\
    \oneres{} & 1/1& 1/2  & 1/0 \\
    \final{} & 1/1  & 2/1  & 1/0  \\
    \bottomrule
    \end{tabular}%
  \caption{\normalfont Approximate number of sequential/random access per swap on each round for the five implementations of random permutation.}
  \label{tab:rp-count}%
  \end{minipage}

  \centering
%\vspace{-1em}
  \begin{minipage}[h]{0.4\textwidth}
    \small
    \begin{tabular}{lcccc}
    \toprule
    Additional space &  0.4\% & 1\%   & 2\%   & 4\% \\
    Running time (ms) & 537   & 425   & 411   & 388 \\
    \bottomrule
    \end{tabular}%
  \end{minipage}\hspace{1em}
  \begin{minipage}[h]{0.4\textwidth}
  \vspace{1em}
  \caption{\normalfont Running time with different restrictions on additional space for \final{} on 72 cores with hyper-threading.  The input is 100 million 64-bit integers.\label{tab:rp-additional-space}}
  \end{minipage}


%\vspace{1em}

